A Performance Study of LLM-Generated Code on Leetcode

This study evaluates the efficiency of code generation by Large Language Models (LLMs) and measures their performance against human-crafted solutions using a dataset from Leetcode. We compare 18 LLMs, considering factors such as model temperature and success rate, and their impact on code performance. This research introduces a novel method for measuring and comparing the speed of LLM-generated code, revealing that LLMs produce code with comparable performance, irrespective of the adopted LLM. We also find that LLMs are capable of generating code that is, on average, more efficient than the code written by humans. The paper further discusses the use of Leetcode as a benchmarking dataset, the limitations imposed by potential data contamination, and the platform's measurement reliability. We believe that our findings contribute to a better understanding of LLM capabilities in code generation and set the stage for future optimizations in the field.

==> Review.tex <==
\newpage
\appendix
\section{Submission reviews and commentary}
Criteria for selecting models are not specified: since I don’t see any LLM model from the GPT family, it makes me wonder what your criteria are for selecting models. It's mentioned as "18 popular LLMs from Hugging Face." You should specify whether popularity is based on the number of likes, downloads, or reported Pass@k values. 

-> We did not use any OpenAI's GPT models (except GitHub Copilot), because they cost too much money to use in our experiment. We also did not use other open source GPT models such as GPT-NeoX because they were not trained for code generation tasks. The models were selected on their ability to generate code (Evaluated using HumanEval, MBPP, or another) and on the number of likes and downloads.
\note{Added in paper}.
\medskip

For better reproducibility, in gathering canonical solutions, it would be helpful to specify the threshold for selecting solutions among the most upvoted ones.

-> When gathering canonical solutions from Leetcode users' questions, we selected the one with the most upvotes.\note{Added in paper}
\medskip

Some figures are a bit unclear: I think the titles of the axes in Figure 7 are not correct.

-> \todo{The titles are correct, but unclear, maybe we should explain it better ?} 
\medskip

Also, the given example on line 722 does not match the data in Figure 6.

-> It has been corrected
\medskip


Following the validation process, when it is mentioned that “the initial set of 210, 120 generated solutions was pruned down to 7481 (3.6\%) valid solutions remaining across the 18 LLMs.” I wondered how many valid solutions would remain per each model. My concern is that this validation process might invalidate all solutions from one model at least for some problems. Have you considered any steps to prevent this?

-> We could prevent the problem by generating more solutions, which would increase the chance of a model generating correct solutions for a problem, but this would be very costly in time and resources. Instead, we deal with this issue by taking the incomplete coverage of problems of each model into account in our comparisons. The pairwise comparisons that we used, compare two models exclusively on the problems they both solved. While we are still limited by the fact that some models can't generate solutions for certain problems, we can still compare models on the same grounds.\todo{Put in paper ?}
\medskip

The paper identifies a significant challenge related to data contamination in using Leetcode problems as a dataset for evaluating LLMs, which may limit the accuracy of performance evaluations and reproducibility of the study.

-> Yeah...
\medskip

The study heavily relies on Leetcode's test suite and its online judge system as a crucial component of its methodology for both validating the generated solutions and benchmarking their performance. This may introduce biases or limitations in the evaluation process

-> Yeah...
\medskip

The focus on algorithmic problems from Leetcode may limit the generalizability of the study's findings to other programming fields or types of code generation tasks, reducing the applicability of the results in broader contexts.

-> Yeah...
\medskip

While the paper acknowledges this challenge of data contamination issue related to using Leetcode problems as a dataset, it could further elaborate on how the study addresses or mitigates this issue and whether there are any remaining uncertainties or limitations in the research methodology or findings.

-> \todo{Explain} 
Normally, all is already said in terms of how the issues are addressed/mitigated. We mitigated it by using newer problems that were not present in the training datasets of the LLMs.
\medskip

While the paper discusses implications for SE research and practice, it could provide more explicit examples or scenarios to illustrate how its contributions could be applied in real-world SE contexts.

-> For example : When selecting an LLM for code generation tasks such as GitHub Copilot, the performance of the code may be an important concern. With our study, developers can have the comfort of knowing that LLMs do not differ in the performance of their generated code. \todo{Add to paper. Where ?}
\medskip


Limited discussion on potential biases or limitations in the evaluation process.

-> The focus on algorithmic problems from Leetcode may limit the generalizability of the study's findings to other programming fields or types of code generation tasks, reducing the applicability of the results in broader contexts. Using Leetcode's test suite and judge system may introduce biases or limitations in the evaluation process. \note{This was just a previous critic}
\medskip

Insufficient exploration of uncertainties or gaps in the research findings.
 
-> \todo{J'ai pas compris}
\medskip



The paper lacks novelty and an adequate review of related works.
The contributions are limited.

The empirical nature of this study is undermined by its similarity to existing work (see comments on novelty). Besides, the authors select problems of varying difficulty from Leetcode—easy, medium, hard. However, the paper does not analyze their results across these levels. Instead, it concludes based on the number of problems in RQ2.

-> 
Concerning the difficulty, we cannot make any conclusions on the effect of difficulty on the performance of LLM-generated code. This is due to the fact that because of the low number of valid generations, we compare LLMs on a small set of problems (< 10 problems), that are more often than not, easy problems. However, we believe that because LLMs-generated code showed no differences in performance accross LLMs, the difficulty of the problems should not be a factor of performance when comparing LLMs. This should be explored in further research. \todo{Add in paper}
\medskip

The paper's claimed novelty is questionable. Despite this paper's claim that no prior research has evaluated the performance of LLM-generated codes, numerous studies exist in this area investigating different aspects of performances, such as [1,2,3]. Some of this paper's content, including the approach to evaluating data leakage and comparing LLM-generated and human solutions on Leetcode and some findings, is similar to the work of Tian et al. [2]. I suggest it is essential for the authors to introduce the related works and clearly distinguish their contributions (specific aspects of performance).


[1] Liu, Jiawei, et al. "Is your code generated by chatgpt really correct? rigorous evaluation of large language models for code generation." Advances in Neural Information Processing Systems 36 (2024).

-> In the paper from Liu \etal, the researchers evaluated 26 populars LLMs including some present in our study (CodeLLama, StarCoder, CodeGen, CodeGen2, SantaCoder) on the correctness of the generated code. Their contributions consisted of studying and improving code benchmarks for LLMs. Whereas in our study, we propose a new benchmarking method for evaluating the performance of the code generated by LLMs, and study the usability of Leetcode as a benchmark.
\medskip


[2] Tian, Haoye, et al. "Is ChatGPT the Ultimate Programming Assistant--How far is it?." arXiv preprint arXiv:2304.11938 (2023).

-> In the paper from Tian \etal, specifically in their contributions concerning code generation, the researchers evaluated ChatGPT, Codex and CodeGen on their ability to generate code using Leetcode. They also noticed the effects of the data-contamination issue on Leetcode and compared the performance of the LLM-generated solutions. However, we observe multiple issues with their methods. First, they measured the performance of their solution using the Leetcode ranking, which we showed was unreliable because of the dependance of the measures from the previous measures, and because the Leetcode time on which the ranking depends is also less precise than traditional measuring methods. Then, the method for generating the solutions was subpar. For generating solutions using Codex and CodeGen, they used the default temperature of the generations methods, that is, 1, which is known to provide worse results, especially when generating only one solution per problem~\cite{chenEvaluatingLargeLanguage2021}. Consequently, the fact that they only did one generation per problem and model and at a fixed temperature prevents any fair comparison between ChatGPT, Codex and CodeGen, thus hindering the validity of their conclusions concerning the correctness and performance of the generated code.

-> We only interest ourselves in the code generation part of the paper.
\medskip

[3]Vaithilingam, Priyan, Tianyi Zhang, and Elena L. Glassman. "Expectation vs. experience: Evaluating the usability of code generation tools powered by large language models." Chi conference on human factors in computing systems extended abstracts. 2022.

-> In the research done by Vaithilingam \etal, they studied how programmers use and perceive GitHub Copilot by conducting a within-subjects user study. The participants had to complete a programming task either with or without using GitHub Copilot. Their study is very different from ours, as they studied a single LLM in the form of a pair-programming code assistant, where we studied the performance of the code of multiple LLMs not led by any human.
\medskip

The paper is well-written and structured effectively. However, the authors need to better articulate how their work extends beyond existing research and clarify their unique contributions.

-> Our unique contributions are :We evaluated Leetcode as a dataset and benchmark platform for evaluating LLMs. While Leetcode has been used in the past, its usability for evaluating LLMs was seldom put in question (for instance, its time ranking). We evaluated the performance of the code generated by different LLMs, using a novel method. We are the first work that we know of that aims to rigorously compare LLM's code performance (We're not including [2] nor Yetistiren et al as it was not the main focus of their studies, and the measures were done in a not so rigorous way), and explore how it changes across LLMs and temperature


==> latexmk <==
# Settings
$xdvipdfmx = "xdvipdfmx -z 6 -i dvipdfmx-unsafe.cfg -o %D %O %S";

# Workaround to allow pstricks transparency (https://github.com/overleaf/issues/issues/3449)
$dvipdf = "dvipdf -dNOSAFER -dALLOWPSTRANSPARENCY %O %S %D";

###############################
# Post processing of pdf file #
###############################

$compiling_cmd = "internal overleaf_pre_process %T %D";
$success_cmd = "internal overleaf_post_process %T %D";
$failure_cmd = $success_cmd;

# equivalent to -gt option. Used to prevent latexmk from skipping recompilation
# of output.log and output.pdf
$go_mode = 3;

# equivalent to -bibtex option. Run bibtex unconditionally when bbl files are
# out of date.
$bibtex_use = 2;

my $ORIG_PDF_AGE;

sub overleaf_pre_process {
    my $source_file = $_[0];
    my $output_file = $_[1];

    # get age of existing pdf if present
    $ORIG_PDF_AGE = -M $output_file
}

sub overleaf_post_process {
    my $source_file = $_[0];
    my $output_file = $_[1];
    my $source_without_ext = $source_file =~ s/\.tex$//r;
    my $output_without_ext = $output_file =~ s/\.pdf$//r;

    # Look for a knitr concordance file
    my $concordance_file = "${source_without_ext}-concordance.tex";
    if (-e $concordance_file) {
        print "Patching synctex file for knitr...\n";
        system("patchSynctex.R", $source_without_ext, $output_without_ext);
    }

    # Return early if pdf file doesn't exist or wasn't updated
    my $NEW_PDF_AGE = -M $output_file;
    return if !defined($NEW_PDF_AGE);
    return if defined($ORIG_PDF_AGE) && $NEW_PDF_AGE == $ORIG_PDF_AGE;

    # Figure out where qpdf is
    $qpdf //= "/usr/bin/qpdf";
    $qpdf = $ENV{QPDF} if defined($ENV{QPDF}) && -x $ENV{QPDF};
    return if ! -x $qpdf;
    $qpdf_opts //= "--linearize --newline-before-endstream";
    $qpdf_opts = $ENV{QPDF_OPTS} if defined($ENV{QPDF_OPTS});

    # Run qpdf
    my $optimised_file = "${output_file}.opt";
    system($qpdf, split(' ', $qpdf_opts), $output_file, $optimised_file);
    $qpdf_exit_code = ($? >> 8);
    print "qpdf exit code=$qpdf_exit_code\n";

    # Replace the output file if qpdf was successful
    # qpdf returns 0 for success, 3 for warnings (output pdf still created)
    return if !($qpdf_exit_code == 0 || $qpdf_exit_code == 3);
    print "Renaming optimised file to $output_file\n";
    rename($optimised_file, $output_file);

    print "Extracting xref table for $output_file\n";
    my $xref_file = "${output_file}xref";
    system("$qpdf --show-xref ${output_file} > ${xref_file}");
    $qpdf_xref_exit_code = ($? >> 8);
    print "qpdf --show-xref exit code=$qpdf_xref_exit_code\n";
}

##############
# Glossaries #
##############
add_cus_dep( 'glo', 'gls', 0, 'glo2gls' );
add_cus_dep( 'acn', 'acr', 0, 'glo2gls');  # from Overleaf v1
sub glo2gls {
    system("makeglossaries $_[0]");
}

#############
# makeindex #
#############
@ist = glob("*.ist");
if (scalar(@ist) > 0) {
    $makeindex = "makeindex -s $ist[0] %O -o %D %S";
}

################
# nomenclature #
################
add_cus_dep("nlo", "nls", 0, "nlo2nls");
sub nlo2nls {
        system("makeindex $_[0].nlo -s nomencl.ist -o $_[0].nls -t $_[0].nlg");
}

#########
# Knitr #
#########
add_cus_dep( 'Rtex', 'tex', 0, 'do_knitr');
add_cus_dep( 'Rnw', 'tex', 0, 'do_knitr');
sub do_knitr {
    Run_subst(qq{Rscript -e '
        library("knitr");
        opts_knit\$set(concordance=T);
        knitr::knit(%S, output=%D);
        '}
    );
}

##########
# feynmf #
##########
push(@file_not_found, '^feynmf: Files .* and (.*) not found:$');
add_cus_dep("mf", "tfm", 0, "mf_to_tfm");
sub mf_to_tfm { system("mf '\\mode:=laserjet; input $_[0]'"); }

push(@file_not_found, '^feynmf: Label file (.*) not found:$');
add_cus_dep("mf", "t1", 0, "mf_to_label1");
sub mf_to_label1 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t1"); }
add_cus_dep("mf", "t2", 0, "mf_to_label2");
sub mf_to_label2 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t2"); }
add_cus_dep("mf", "t3", 0, "mf_to_label3");
sub mf_to_label3 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t3"); }
add_cus_dep("mf", "t4", 0, "mf_to_label4");
sub mf_to_label4 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t4"); }
add_cus_dep("mf", "t5", 0, "mf_to_label5");
sub mf_to_label5 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t5"); }
add_cus_dep("mf", "t6", 0, "mf_to_label6");
sub mf_to_label6 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t6"); }
add_cus_dep("mf", "t7", 0, "mf_to_label7");
sub mf_to_label7 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t7"); }
add_cus_dep("mf", "t8", 0, "mf_to_label8");
sub mf_to_label8 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t8"); }
add_cus_dep("mf", "t9", 0, "mf_to_label9");
sub mf_to_label9 { system("mf '\\mode:=laserjet; input $_[0]' && touch $_[0].t9"); }

##########
# feynmp #
##########
push(@file_not_found, '^dvipdf: Could not find figure file (.*); continuing.$');
add_cus_dep("mp", "1", 0, "mp_to_eps");
sub mp_to_eps {
    system("mpost $_[0]");
    return 0;
}

#############
# asymptote #
#############

sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

#############
# metapost  #  # from Overleaf v1
#############
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
    my $file = $_[0];
    my ($name, $path) = fileparse($file);
    pushd($path);
    my $return = system "mpost $name";
    popd();
    return $return;
}

##########
# chktex #
##########
unlink 'output.chktex' if -f 'output.chktex';
if (defined $ENV{'CHKTEX_OPTIONS'}) {
    use File::Basename;
    use Cwd;

    # identify the main file
    my $target = $ARGV[-1];
    my $file = basename($target);

    if ($file =~ /\.tex$/) {
        # change directory for a limited scope
        my $orig_dir = cwd();
        my $subdir = dirname($target);
        chdir($subdir);
        # run chktex on main file
        $status = system("/usr/local/bin/run-chktex.sh", $orig_dir, $file);
        # go back to original directory
        chdir($orig_dir);

        # in VALIDATE mode we always exit after running chktex
        # otherwise we exit if EXIT_ON_ERROR is set

        if ($ENV{'CHKTEX_EXIT_ON_ERROR'} || $ENV{'CHKTEX_VALIDATE'}) {
            # chktex doesn't let us access the error info via exit status
            # so look through the output
            open(my $fh, "<", "output.chktex");
            my $errors = 0;
            {
                local $/ = "\n";
                while(<$fh>) {
                    if (/^\S+:\d+:\d+: Error:/) {
                        $errors++;
                        print;
                    }
                }
            }
            close($fh);
            exit(1) if $errors > 0;
            exit(0) if $ENV{'CHKTEX_VALIDATE'};
        }
    }
}


==> leetcode_results.tex <==


\begin{tabular}{@{}lccccccccccc@{}}
\toprule
Model & \begin{tabular}[c]{@{}c@{}}English-\\ trained\end{tabular} & \multicolumn{4}{c}{pass@1} & \multicolumn{4}{c}{pass@10} & \begin{tabular}[c]{@{}c@{}}MNRT-\\Glob\end{tabular} & \begin{tabular}[c]{@{}c@{}}MNRT-\\Best\end{tabular} \\ \midrule
 &  & Avg. & Easy & Med & Hard & Avg. & Easy & Med & Hard &  &  \\
 \cmidrule(lr){3-6} \cmidrule(lr){7-10}
Codex & \checkmark & \textbf{.823} & \textbf{.954} & \textbf{.929} & \textbf{.602} & \textbf{.960} & \textbf{1.0} & \textbf{.990} & \textbf{.900} & 0.111 & \textbf{-0.130} \\
GitHub Copilot & \checkmark & .745 & .856 & .832 & .547 & .917 & .947 & .952 & .850 & \textbf{-0.163} & 0.054 \\
CodeGen-Mono 6B &  \checkmark & .548 & .783 & .697 & .168 & .763 & .958 & .952 & .380 & -0.002 & -0.010 \\
CodeGen-Mono 2B &  \checkmark & .472 & .692 & .586 & .144 & .707 & .947 & .886 & .290 & -0.084 & -0.083 \\
SantaCoder &   & .202 & .379 & .204 & .031 & .400 & .684 & .486 & .070 & 0.03 & 0.135 \\
CodeGen-Mono 350M & \checkmark & .191 & .333 & .240 & .011 & .383 & .621 & .505 & .050 & 0.076 & 0.055 \\
CodeT5 (large-ntp-py) &   & .087 & .217 & .047 & .011 & .200 & .432 & .181 & .030 & 0.006 & 0.101 \\
InCoder 6B &  & .076 & .184 & .053 & .004 & .183 & .400 & .152 & .040 & -0.163 & 0.200 \\
InCoder 1B &   & .023 & .060 & .018 & .005 & .087 & .200 & .067 & .020 & N/A & N/A \\
CodeParrot &   & .004 & .008 & .005 & .002 & .023 & .032 & .029 & .020 & N/A & N/A \\
CodeT5 (large) &  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & N/A & N/A \\ \bottomrule
\end{tabular}


==> leetcode_results_only_validity.tex <==
\begin{tabular}{@{}ccccccc@{}}
\toprule
Model & Model family & Open-source & Parameters (B) & \begin{tabular}[c]{@{}c@{}}Trained on\\ English text\end{tabular} & pass@1 & pass@10 \\ \midrule
codex               & Codex      & No  & 11   & Yes & 0.823 & 0.960 \\
copilot             & Codex      & No  & 11   & Yes & 0.745 & 0.917 \\
codegen-6B-mono     & Codegen    & Yes & 6    & Yes & 0.548 & 0.763 \\
codegen-2B-mono     & Codegen    & Yes & 2    & Yes & 0.472 & 0.707 \\
santacoder          & Santacoder & Yes & 1.1  & No  & 0.202 & 0.400 \\
codegen-350M-mono   & Codegen    & Yes & 0.35 & Yes & 0.191 & 0.383 \\
codet5-large-ntp-py & CodeT5     & Yes & 0.77 & No  & 0.087 & 0.200 \\
incoder-6B          & Incoder    & Yes & 6    & No  & 0.076 & 0.183 \\
incoder-1B          & Incoder    & Yes & 1    & No  & 0.023 & 0.087 \\
codeparrot          & Codeparrot & Yes & 1.5  & No  & 0.004 & 0.023 \\
codet5-large        & CodeT5     & Yes & 0.77 & No  & 0.0   & 0.0   \\ \bottomrule
\end{tabular}


==> pairwise_scores.tex <==
\begin{tabular}{ll}
\toprule
    \textbf{\gls{llm} Model} & \textbf{Pairwisescore} \\
    \midrule
    starcoder & \textbf{20.6} \\
    codellama-13b-python & 12.7 \\
    codegen-6B-mono & 11.5 \\
    wizardcoder-python-7B & 6.6 \\
    codellama-13b-instruct & 1.7 \\
    codellama-7b-instruct & -1.4 \\
    codellama-7b-python & -4.5 \\
    codegen25-7B-mono & -5.2 \\
    codegen-2B-mono & -8.0 \\
    replit-code-v1-3b & -13.7 \\
    codegen25-7b-instruct & -25.1 \\
\end{tabular}


==> pass_at_k.tex <==
\begin{tabular}{@{}lcccccccc@{}}
\toprule
Model & \multicolumn{4}{c}{pass@1} & \multicolumn{4}{c}{pass@10} \\ 
\midrule
    & Avg. & Easy & Med & Hard & Avg. & Easy & Med & Hard\\
    \cmidrule(lr){2-5} \cmidrule(lr){6-9}

GitHub Copilot & .745/.063 & .856/.250 & .832/.053 & .547/.005 & .917/.137 & .947/.482 & .952/.125 & .850/.045 \\
CodeGen-Mono 6B & .548/.031 & .783/.164 & .697/.003 & .168/.007 & .763/.077 & .958/.357 & .952/.029 & .380/.045 \\
CodeGen-Mono 2B & .472/.038 & .692/.136 & .586/.003 & .144/0 & .707/.103 & .947/.339 & .886/.029 & .290/0 \\
SantaCoder  & .297/.015 & .383/.055 & .202/.003 & .025/.002 & .588/.064 & .688/.196 & .486/.029 & .061/0.023 \\
CodeGen-Mono 350M & .191 & .333 & .240 & .011 & .383 & .621 & .505 & .050 \\
InCoder 6B & .076 & .184 & .053 & .004 & .183 & .400 & .152 & .040 \\
InCoder 1B & .023 & .060 & .018 & .005 & .087 & .200 & .067 & .020\\
CodeParrot & .004 & .008 & .005 & .002 & .023 & .032 & .029 & .020\\
\end{tabular}

